EXCESS workshop: Descriptions of rising low-energy spectra

Many low-threshold experiments observe sharply rising event rates of yet unknown origins below a few hundred eV, and larger than expected from known backgrounds. Due to the significant impact of this excess on the dark matter or neutrino sensitivity of these experiments, a collective effort has been started to share the knowledge about the individual observations. For this, the EXCESS Workshop was initiated. In its first iteration in June 2021, ten rare event search collaborations contributed to this initiative via talks and discussions. The contributing collaborations were CONNIE, CRESST, DAMIC, EDELWEISS, MINER, NEWS-G, NUCLEUS, RICOCHET, SENSEI and SuperCDMS. They presented data about their observed energy spectra and known backgrounds together with details about the respective measurements. In this paper, we summarize the presented information and give a comprehensive overview of the similarities and differences between the distinct measurements. The provided data is furthermore publicly available on the workshop's data repository together with a plotting tool for visualization.

==> CRESST_authors.tex <==
\author{
  G.~Angloher\thanksref{addrMPI}\and
  G.~Benato\thanksref{addrLNGS}\and
  A.~Bento\thanksref{addrMPI,addrCoimbra}\and 
  A.~Bertolini\thanksref{addrMPI}\and 
  R.~Breier\thanksref{addrBratislava}\and
  C.~Bucci\thanksref{addrLNGS}\and 
  L.~Canonica\thanksref{addrMPI}\and 
  A.~D'Addabbo\thanksref{addrLNGS}\and
  S.~Di~Lorenzo\thanksref{addrLNGS}\and
  L.~Einfalt\thanksref{addrHEPHY,addrAI}\and
  A.~Erb\thanksref{addrTUM,addrWMI}\and
  F.~v.~Feilitzsch\thanksref{addrTUM}\and 
  N.~Ferreiro~Iachellini\thanksref{addrMPI}\and
  S.~Fichtinger\thanksref{addrHEPHY}\and
  D.~Fuchs\thanksref{addrMPI}\and 
  A.~Fuss\thanksref{addrHEPHY,addrAI}\and
  A.~Garai\thanksref{addrMPI}\and 
  V-M.~Ghete\thanksref{addrHEPHY}\and
  P.~Gorla\thanksref{addrLNGS}\and
  S.~Gupta\thanksref{addrHEPHY}\and 
  D.~Hauff\thanksref{addrMPI}\and 
  M.~Ješkovsk\'y\thanksref{addrBratislava}\and
  J.~Jochum\thanksref{addrTUE}\and
  M.~Kaznacheeva\thanksref{addrTUM}\and
  A.~Kinast\thanksref{addrTUM}\and
  H.~Kluck\thanksref{addrHEPHY}\and
  H.~Kraus\thanksref{addrOxford}\and 
  A.~Langenk\"amper\thanksref{addrTUM}\and 
  M.~Mancuso\thanksref{addrMPI}\and
  L.~Marini\thanksref{addrLNGS}\and 
  V.~Mokina\thanksref{addrHEPHY}\and
  A.~Nilima\thanksref{addrMPI}\and 
  M.~Olmi\thanksref{addrLNGS}\and
  T.~Ortmann\thanksref{addrTUM}\and
  C.~Pagliarone\thanksref{addrLNGS,addrCASS}\and
  V.~Palušov\'a\thanksref{addrBratislava}\and
  L.~Pattavina\thanksref{addrTUM,addrGSSI}\and
  F.~Petricca\thanksref{addrMPI}\and 
  W.~Potzel\thanksref{addrTUM}\and 
  P.~Povinec\thanksref{addrBratislava}\and
  F.~Pr\"obst\thanksref{addrMPI}\and
  F.~Pucci\thanksref{addrMPI}\and 
  F.~Reindl\thanksref{addrHEPHY,addrAI} \and
  J.~Rothe\thanksref{addrTUM}\and 
  K.~Sch\"affner\thanksref{addrMPI}\and 
  J.~Schieck\thanksref{addrHEPHY,addrAI}\and 
  D.~Schmiedmayer\thanksref{addrHEPHY,addrAI}\and
  S.~Sch\"onert\thanksref{addrTUM}\and 
  C.~Schwertner\thanksref{addrHEPHY,addrAI}\and
  M.~Stahlberg\thanksref{addrMPI}\and 
  L.~Stodolsky\thanksref{addrMPI}\and 
  C.~Strandhagen\thanksref{addrTUE}\and
  R.~Strauss\thanksref{addrTUM}\and
  I.~Usherov\thanksref{addrTUE}\and
  F.~Wagner\thanksref{addrLNGS}\and 
  M.~Willers\thanksref{addrTUM}\and 
  V.~Zema\thanksref{addrMPI}\and
(CRESST Collaboration)
}

\institute
{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany \label{addrMPI} \and
INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy \label{addrLNGS} \and
Comenius University, Faculty of Mathematics, Physics and Informatics, 84248 Bratislava, Slovakia \label{addrBratislava} \and
Physik-Department and Excellence Cluster Universe, Technische Universit\"at M\"unchen, D-85747 Garching, Germany \label{addrTUM} \and
Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, A-1050 Wien, Austria\label{addrHEPHY} \and
Atominstitut, Technische Universit\"at Wien, A-1020 Wien, Austria \label{addrAI} \and
Eberhard-Karls-Universit\"at T\"ubingen, D-72076 T\"ubingen, Germany \label{addrTUE} \and
Department of Physics, University of Oxford, Oxford OX1 3RH, United Kingdom \label{addrOxford} \and
also at: Departamento de Fisica, Universidade de Coimbra, P3004 516 Coimbra, Portugal \label{addrCoimbra} \and
also at: GSSI-Gran Sasso Science Institute, I-67100 L'Aquila, Italy \label{addrGSSI} \and
also at: Walther-Mei\ss ner-Institut f\"ur Tieftemperaturforschung, D-85748 Garching, Germany \label{addrWMI} \and
also at: Dipartimento di Ingegneria Civile e Meccanica, Universitá degli Studi di Cassino e del Lazio Meridionale, I-03043 Cassino, Italy\label{addrCASS}
}



==> DAMIC_author_list.tex <==
%DAMIC at SNOLAB author list

\author{A.~Aguilar-Arevalo} 
\affiliation{Universidad Nacional Aut{\'o}noma de M{\'e}xico, Mexico City, Mexico} 

\author{D.~Amidei}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, Michigan, USA}  

\author{D.~Baxter}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois, USA}

\author{G.~Cancelo}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois, USA}

\author{B.A.~Cervantes Vergara}
\affiliation{Universidad Nacional Aut{\'o}noma de M{\'e}xico, Mexico City, Mexico} 

\author{A.E.~Chavarria}
\affiliation{Center for Experimental Nuclear Physics and Astrophysics, University of Washington, Seattle, Washington, USA}

\author{ J.C.~D'Olivo}
\affiliation{Universidad Nacional Aut{\'o}noma de M{\'e}xico, Mexico City, Mexico} 

\author{J.~Estrada}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois, USA}

\author{F.~Favela-Perez}
\affiliation{Universidad Nacional Aut{\'o}noma de M{\'e}xico, Mexico City, Mexico} 

\author{R.~Ga\"ior}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes \'Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{Y.~Guardincerri}
\thanks{Deceased January 2017}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois, USA}

\author{E.W.~Hoppe}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, Washington, USA} 

\author{ T.W.~Hossbach}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, Washington, USA} 

\author{B.~Kilminster}
\affiliation{Universit{\"a}t Z{\"u}rich Physik Institut, Zurich, Switzerland }

\author{I.~Lawson}
\affiliation{SNOLAB, Lively, Ontario, Canada }

\author{S.J.~Lee}
\affiliation{Universit{\"a}t Z{\"u}rich Physik Institut, Zurich, Switzerland }

\author{A.~Letessier-Selvon}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes \'Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{A.~Matalon}
\affiliation{Kavli Institute for Cosmological Physics and The Enrico Fermi Institute, The University of Chicago, Chicago, Illinois, USA}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes \'Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{P.~Mitra}
\affiliation{Center for Experimental Nuclear Physics and Astrophysics, University of Washington, Seattle, Washington, USA}

\author{C.T.~Overman}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, Washington, USA} 

\author{A.~Piers}
\affiliation{Center for Experimental Nuclear Physics and Astrophysics, University of Washington, Seattle, Washington, USA}

\author{P.~Privitera}
\affiliation{Kavli Institute for Cosmological Physics and The Enrico Fermi Institute, The University of Chicago, Chicago, Illinois, USA}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes \'Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{K.~Ramanathan}
\affiliation{Kavli Institute for Cosmological Physics and The Enrico Fermi Institute, The University of Chicago, Chicago, Illinois, USA}
\affiliation{Division of Physics, Mathematics, & Astronomy, California Institute of Technology, Pasadena, California, USA}

\author{J.~Da~Rocha}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes \'Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{Y.~Sarkis}
\affiliation{Universidad Nacional Aut{\'o}noma de M{\'e}xico, Mexico City, Mexico}

\author{M.~Settimo}
\affiliation{SUBATECH, CNRS-IN2P3, IMT Atlantique, Universit\'e de Nantes, Nantes, France}

\author{R.~Smida}
\affiliation{Kavli Institute for Cosmological Physics and The Enrico Fermi Institute, The University of Chicago, Chicago, Illinois, USA}

\author{R.~Thomas}
\affiliation{Kavli Institute for Cosmological Physics and The Enrico Fermi Institute, The University of Chicago, Chicago, Illinois, USA}

\author{J.~Tiffenberg}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois, USA}

\author{M.~Traina}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes \'Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{A.L.~Virto}
\affiliation{Instituto de F\'isica de Cantabria (IFCA), CSIC--Universidad de Cantabria, Santander, Spain}

\collaboration{DAMIC Collaboration}


==> EDELWEISS_authors.tex <==
Julien Billard
Jules Gascon
Elsa Guy
Hugues Lattaud

Univ Lyon, Universit\'e Lyon 1, CNRS/IN2P3, IP2I-Lyon, F-69622, Villeurbanne, France

==> NEWSG_author_list.tex <==
\author[labelQueens_DMME]{L.~Balogh}
\author[labelGrenoble]{C.~Beaufort}
\author[labelQueens]{A.~Brossard}
\author[labelQueens_DMME]{J.-F.~Caron}
\author[labelQueens]{M.~Chapellier}
\author[labelQueens]{J.-M.~Coquillat}
\author[labelRMC]{E.~C.~Corcoran}
\author[labelQueens]{S.~Crawford}
\author[labelGrenoble]{A.~Dastgheibi-Fard}
\author[labelAlberta]{Y.~Deng}
\author[labelQueens]{K.~Dering}
\author[labelAlberta]{D.~Durnford}
\author[labelAlberta]{C.~Garrah}
\author[labelQueens]{G.~Gerbier}
\author[labelCEA]{I.~Giomataris}
\author[labelQueens]{G.~Giroux}
\author[labelLaurentian,labelSNOLAB,labelMcDonald]{P.~Gorel}
\author[labelCEA]{M.~Gros}
\author[labelQueens]{P.~Gros}
\author[labelGrenoble]{O.~Guillaudin}
\author[labelPNNL]{E.~W.~Hoppe}
\author[labelBirmingham]{I.~Katsioulas}
\author[labelRMC]{F.~Kelly}
\author[labelBirmingham]{P.~Knights}
\author[labelLaurentian,labelSNOLAB,labelMcDonald]{S.~Langrock}
\author[labelSubatech]{P.~Lautridou}
\author[labelBirmingham]{I.~Manthos}
\author[labelQueens]{R.~D.~Martin}
\author[labelBirmingham]{J.~Matthews}
\author[labelCEA]{J.-P.~Mols}
\author[labelGrenoble]{J.-F.~Muraz}
\author[labelBirmingham]{T.~Neep}
\author[labelBirmingham]{K.~Nikolopoulos}
\author[labelAlberta]{P.~O'Brien}
\author[labelAlberta]{M.-C.~Piro}
\author[labelQueens]{N.~Rowe}
\author[labelGrenoble]{D.~Santos}
\author[labelQueens]{G.~Savvidis}
\author[labelThessaloniki]{I.~Savvidis}
\author[labelSubatech]{F.~A.~Vazquez~de~Sola~Fernandez}
\author[labelQueens]{M.~Vidal}
\author[labelBirmingham]{R.~Ward}
\author[labelGrenoble]{M.~Zampaolo}

\address[labelQueens_DMME]{Department of Mechanical and Materials Engineering, Queen’s University, Kingston, Ontario K7L 3N6, Canada}
\address[labelQueens]{Department of Physics, Engineering Physics \& Astronomy, Queen’s University, Kingston, Ontario K7L 3N6, Canada}
\address[labelGrenoble]{LPSC, Université Grenoble-Alpes, CNRS/IN2P3, Grenoble 38026, France}
\address[labelRMC]{Chemistry \& Chemical Engineering Department, Royal Military College of Canada, Kingston, Ontario K7K 7B4, Canada}
\address[labelAlberta]{Department of Physics, University of Alberta, Edmonton, Alberta, T6G 2R3, Canada}
\address[labelCEA]{IRFU, CEA, Université Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\address[labelLaurentian]{Department of Physics and Astronomy, Laurentian University, Sudbury, Ontario, P3E 2C6, Canada}
\address[labelSNOLAB]{SNOLAB, Lively, Ontario, P3Y 1N2, Canada}
\address[labelMcDonald]{Arthur B. McDonald Canadian Astroparticle Physics Research Institute, Queen’s University, Kingston, ON, K7L 3N6, Canada}
\address[labelSubatech]{SUBATECH, IMT-Atlantique/CNRS-IN2P3/Université de Nantes, Nantes 44307, France}
\address[labelPNNL]{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\address[labelBirmingham]{School of Physics and Astronomy, University of Birmingham, Birmingham B15 2TT, United Kingdom}
\address[labelThessaloniki]{Aristotle University of Thessaloniki, Thessaloniki 54124, Greece}


==> SENSEI_authors.tex <==
\author{Prakruth Adari}
\affiliation{\normalsize\it 
C.N.~Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, NY 11794, USA}

 \author{Yonatan Ben Gal}
 \affiliation{\normalsize\it 
 School of Physics and Astronomy, 
 Tel-Aviv University, Tel-Aviv 69978, Israel}

 \author{Itay M. Bloch}
 \affiliation{\normalsize\it 
 School of Physics and Astronomy, 
 Tel-Aviv University, Tel-Aviv 69978, Israel}

\author{Mariano Cababie}
\affiliation{\normalsize\it 
Department of Physics, FCEN, University of Buenos Aires and IFIBA, CONICET, Buenos Aires, Argentina}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Gustavo Cancelo}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Luke Chaplinsky}
\affiliation{\normalsize\it 
Amherst Center for Fundamental Interactions, University of Massachusetts, Amherst, MA 01003-9337, USA}
\affiliation{\normalsize\it 
Department of Physics, University of Massachusetts, Amherst, MA 01003-9337, USA}

\author{Fernando Chierchie}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Michael Crisler}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Alex Drlica-Wagner}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}
\affiliation{\normalsize\it Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{\normalsize\it  Department of Astronomy and Astrophysics, University of Chicago, Chicago IL 60637, USA}

\author{Rouven Essig}
\affiliation{\normalsize\it 
C.N.~Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, NY 11794, USA}

 \author{Juan Estrada}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Erez Etzion}
\affiliation{\normalsize\it 
 School of Physics and Astronomy, 
 Tel-Aviv University, Tel-Aviv 69978, Israel}

\author{Guillermo Fernandez Moroni}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Daniel Gift}
\affiliation{\normalsize\it 
C.N.~Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, NY 11794, USA}
\affiliation{\normalsize\it 
Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794, USA} 

 \author{Yaron Korn}
 \affiliation{\normalsize\it 
 School of Physics and Astronomy, 
 Tel-Aviv University, Tel-Aviv 69978, Israel}

\author{Sravan Munagavalasa}
\affiliation{\normalsize\it 
Kavli Institute for Cosmological Physics and The Enrico Fermi Institute, The University of Chicago, Chicago, IL, USA}

 \author{Aviv Orly}
\affiliation{\normalsize\it 
 School of Physics and Astronomy, 
 Tel-Aviv University, Tel-Aviv 69978, Israel}

\author{Dario Rodrigues}
\affiliation{\normalsize\it 
Department of Physics, FCEN, University of Buenos Aires and IFIBA, CONICET, Buenos Aires, Argentina}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Nathan Saffold}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Aman Singal}
\affiliation{\normalsize\it 
Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794, USA}

 \author{Miguel Sofo Haro}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}
\affiliation{Centro At\'omico Bariloche, CNEA/CONICET/IB, Bariloche, Argentina}

\author{Leandro Stefanazzi}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Javier Tiffenberg}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Sho Uemura}
\affiliation{\normalsize\it 
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA}

\author{Tomer Volansky}
\affiliation{\normalsize\it 
 School of Physics and Astronomy,   
 Tel-Aviv University, Tel-Aviv 69978, Israel}

\author{Tien-Tien Yu}
\affiliation{\normalsize\it 
Department of Physics and Institute for Fundamental Science, University of Oregon, Eugene, Oregon 97403, USA}


==> Skipper-CCD_authors.tex <==
\author{Guillermo Fernandez Moroni}
\affiliation{\normalsize Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}
\author{Fernando Chierchie}
\affiliation{\normalsize Instituto de Inv. en Ing. Eléctrica ``Alfredo Desages'' (IIIE), Dpto. de Ing. Eléctrica y de Computadoras. CONICET and Universidad Nacional del Sur (UNS), Bahía Blanca, Argentina.}
\author{Javier Tiffenberg}
\affiliation{\normalsize Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}
\author{Ana Botti}
\affiliation{\normalsize Department of Physics, FCEN, University of Buenos Aires and IFIBA, CONICET, Buenos Aires, Argentina.}

\author{Mariano Cababie}
\affiliation{\normalsize
Department of Physics, FCEN, University of Buenos Aires and IFIBA, CONICET, Buenos Aires, Argentina.}
\affiliation{\normalsize
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}
\author{Gustavo Cancelo}
\affiliation{\normalsize Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}
\author{Eliana L. Depaoli}
\affiliation{\normalsize CNEA - Gerencia de Área Aplicaciones de la Tecnología Nuclear (GAATN) - Gerencia Química Nuclear y Ciencias de la Salud - Dpto. Metrologia de Radioisotopos - Division Metrologia Cientifica Centro Atómico Ezeiza. }

\author{Juan Estrada}
\affiliation{\normalsize Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}
\author{Stephen E. Holland}
\affiliation{\normalsize
Lawrence Berkeley National Laboratory, One Cyclotron Road, Berkeley, California 94720, USA.}
\author{Dario Rodrigues}
\affiliation{\normalsize
Department of Physics, FCEN, University of Buenos Aires and IFIBA, CONICET, Buenos Aires, Argentina.}
\affiliation{\normalsize
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}
\author{Iván Sidelnik}
\affiliation{\normalsize CONICET y CNEA - Comisión Nacional de Energía Atómica, Departamento de física de neutrones, Centro Atómico Bariloche, Av. Bustillo 9500, Bariloche, Argentina.}
 \author{Miguel Sofo Haro}
\affiliation{\normalsize
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}
\affiliation{\normalsize Centro At\'omico Bariloche, CNEA/CONICET/IB, Bariloche, Argentina.}
\author{Leandro Stefanazzi}
\affiliation{\normalsize
Fermi National Accelerator Laboratory, PO Box 500, Batavia IL, 60510, USA.}
\author{Sho Uemura}
\affiliation{\normalsize
 School of Physics and Astronomy,
 Tel-Aviv University, Tel-Aviv 69978, Israel.}

==> SuperCDMS_endorsing_authors.tex <==
%This file only lists authors that are in addition to Valentina, Sam, and Belina, i.e. only those authors which opted in to endorse the effort.

\author{R.~Bhattacharyya} \affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{R.~Bunker} \affiliation{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\author{J.~Cooley} \affiliation{Department of Physics, Southern Methodist University, Dallas, TX 75275, USA}
\author{P.~Cushman} \affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{S.~Dharani} \affiliation{Institut f{\"u}r Experimentalphysik, Universit{\"a}t Hamburg, 22761 Hamburg, Germany}
\author{E.~Figueroa-Feliciano} \affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{M.~Ghaith} \affiliation{Department of Physics, Queen's University, Kingston, ON K7L 3N6, Canada}
\author{Z.~Hong} \affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{N.A.~Kurinsky} \affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{H.~Meyer~zu~Theenhausen} \affiliation{Institute for Astroparticle Physics (IAP), Karlsruhe Institute of Technology (KIT), 76344, Germany}\affiliation{Institut f{\"u}r Experimentalphysik, Universit{\"a}t Hamburg, 22761 Hamburg, Germany}
\author{E.~Michielin} \affiliation{Department of Physics \& Astronomy, University of British Columbia, Vancouver, BC V6T 1Z1, Canada}\affiliation{TRIUMF, Vancouver, BC V6T 2A3, Canada}
\author{J.L.~Orrell} \affiliation{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\author{R.~Ren} \affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{T.~Saab} \affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA}
\author{J.~Sander} \affiliation{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\author{B.~Schmidt} \affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{M.J.~Wilson} \affiliation{Institute for Astroparticle Physics (IAP), Karlsruhe Institute of Technology (KIT), 76344, Germany}
\author{A.~Zaytsev} \affiliation{Institute for Astroparticle Physics (IAP), Karlsruhe Institute of Technology (KIT), 76344, Germany}\affiliation{Institut f{\"u}r Experimentalphysik, Universit{\"a}t Hamburg, 22761 Hamburg, Germany}

